FacTeR-Check: Semi-automated fact-checking through Semantic Similarity and Natural Language Inference

Our society produces and shares overwhelming amounts of information through Online Social Networks (OSNs). Within this environment, misinformation and disinformation have proliferated, becoming a public safety concern in most countries. Allowing the public and professionals to efficiently find reliable evidences about the factual veracity of a claim is a crucial step to mitigate this harmful spread. To this end, we propose FacTeR-Check, a multilingual architecture for semi-automated fact-checking that can be used for either applications designed for the general public and by fact-checking organisations. FacTeR-Check enables retrieving fact-checked information, unchecked claims verification and tracking dangerous information over social media. This architectures involves several modules developed to evaluate semantic similarity, to calculate natural language inference and to retrieve information from Online Social Networks. The union of all these components builds a semi-automated fact-checking tool able of verifying new claims, to extract related evidence, and to track the evolution of a hoax on a OSN. While individual modules are validated on related benchmarks (mainly MSTS and SICK), the complete architecture is validated using a new dataset called NLI19-SP that is publicly released with COVID-19 related hoaxes and tweets from Spanish social media. Our results show state-of-the-art performance on the individual benchmarks, as well as producing a useful analysis of the evolution over time of 61 different hoaxes.

==> FacTeR-Check arxiv-2/table_hoaxes.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table*}[htb]
\centering
\resizebox{1\textwidth}{!}{%
\begin{tabularx}{1.4\textwidth}{lXXX}

\toprule
\textbf{Id} & \textbf{Hoax (in Spanish)} & \textbf{Hoax (in English)} & \textbf{Fact-checkers} \\ \midrule
1 & La PCR no distingue entre coronavirus y gripe & PCR tests do not distinguish between coronavirus and the flu & Newtral.es \\ \midrule
2 & Las vacunas de ARN-m contra el coronavirus nos transforman en seres transgénicos & mRNA vaccines against coronavirus transform us into transgenic beings & Animal Político, Maldita.es, Newtral.es \\ \midrule
3 & La vacuna contra la COVID-19 se crea con células de fetos abortados & COVID-19 vaccines are made of cells from aborted fetuses & Agencia Ocote, Agência Lupa, Chequeado, ColombiaCheck, Maldita.es, Newtral.es \\ \midrule
4 & Merck asocia las vacunas contra la COVID-19 con un genocidio & Merck associates COVID-19 vaccines with a genocide & Ecuador Chequea, Newtral.es \\ \midrule
5 & Una imagen relaciona la prueba PCR con la destrucción de la glándula pineal en el Antiguo Egipto & An image links PCR tests to the destruction of the pineal gland & Maldita.es \\ \midrule
6 & La vacuna contra la COVID-19 produce parálisis facial & COVID-19 vaccines produce facial paralysis & Chequeado, Newtral.es \\ \midrule
7 & La primera ministra de Australia finge ponerse la vacuna contra la COVID-19 & Australia first minister pretends to get the COVID-19 vaccine & Agência Lupa, La Silla Vacía \\ \midrule
8 & La vacuna contra la COVID-19 produce convulsiones & COVID-19 vaccines produce seizures & Maldita.es, Newtral.es \\ \midrule
9 & Mueren 53 personas en Gibraltar tras ponerse la vacuna contra la COVID-19 & 53 people dead after being vaccinated against COVID-19 in Gibraltar & Maldita.es, Newtral.es \\ \midrule
10 & Detienen en un Lidl de Gijón a 11 personas con COVID-19 & 11 people with COVID-19 arrested in Lidl supermarket in Gijón & Maldita.es, Newtral.es \\ \midrule
11 & Ya no existen las enfermedades respiratorias que no son COVID-19 & Respiratory diseases that are not COVID-19 do not exist anymore & Newtral.es \\ \midrule
12 & La PCR da positivo por nuestros genes endógenos, no por coronavirus & PCR tests positive due to our endogenous genes, not due to coronavirus & Newtral.es \\ \midrule
13 & La ciudad de Rosario (Argentina) para la vacunación por los efectos adversos de la vacuna & The city of Rosario (Argentina) stops vaccination because of the adverse effects of the vaccine & Chequeado, Maldita.es \\ \midrule
14 & La OMS dice que llevar a los niños al colegio sirve como consentimiento para su vacunación & The WHO says that taking our children to school gives consent for their vaccination & Maldita.es \\ \midrule
15 & La definición de pandemia cambió en 2009 por la OMS & The definition of pandemic was changed in 2009 by the WHO & Newtral.es \\ \midrule
16 & Muere una enfermera de Tennessee (Estados Unidos) tras vacunarse contra la COVID-19 & A nurse from Tennessee (United States) died after being vaccinated against COVID-19 & La Silla Vacía, Maldita.es, Newtral.es \\ \midrule
17 & Solo el 6\% de las muertes por coronavirus en Estados Unidos fueron realmente por esta causa & Only 6\% of coronavirus deaths in United States were actually due to this cause & AFP, Agência Lupa, Animal Político, Chequeado, La Silla Vacía \\ \midrule
18 & La PCR da positivo por los exosomas, no por coronavirus & PCR tests positive due to exosomes, not due to coronavirus & Newtral.es \\ \midrule
19 & La mascarilla produce enfermedades neurodegenerativas & Masks produce neurodegenerative diseases & Maldita.es, Newtral.es \\ \midrule
20 & En Países Bajos existe desde 2015 una patente de test de COVID-19 & A patent of COVID-19 test exists in the Netherlands since 2015 & Maldita.es, Newtral.es \\ \midrule
21 & La vacuna contra la COVID-19 causa esterilidad & Pfizer vaccines cause sterility & Animal Político, Chequeado, ColombiaCheck, La Silla Vacía, Maldita.es, Newtral.es \\ \midrule
22 & Un estudio de 2008 financiado por la Comisión Europea ya incluía la COVID-19 & A study funded by the European Commission in 2008 already included COVID-19 & Newtral.es \\ \midrule
23 & Varios vacunados con la vacuna UQ-CSL contra la COVID-19 contraen el VIH & Several COVID-19 vaccinated people with UQ-CSL contracted HIV & Newtral.es \\ \midrule
24 & La vacuna contra la COVID-19 es aún experimental porque está en fase 4 & Vaccines against COVID-19 are still experimental because they are in phase 4 & Animal Político, Maldita.es \\ \midrule
25 & El Banco Mundial tenía planes para la COVID-19 desde 2017 & The World Bank had plans for COVID-19 since 2017 & Animal Político, Aos Fatos, Mala Espina Check \\ \midrule
26 & La vacuna contra la COVID-19 destruye nuestro sistema inmunológico & Vaccines against COVID-19 destroy our immune system & Maldita.es, Newtral.es \\ \midrule
27 & Pirbright Institute patentó la COVID-19 en 2018 & Pirbright Institute patented COVID-19 in 2018 & Maldita.es \\ \midrule
28 & Las gargaras con agua y sal previenen o curan el coronavirus & Gargling with water and salt prevents or cures coronavirus & \#NoComaCuento (La Nación), AFP, Chequeado, ColombiaCheck, Ecuador Chequea, Efecto Cocuyo, El Surtidor, La Silla Vacía, Maldita.es, Spondeo Media, Verificador (La República) \\ \midrule
29 & La dieta alcalina previene o cura el coronavirus & Alcaline diets prevent or cure coronavirus & Agência Lupa, Animal Político, Bolivia Verifica, Chequeado, ColombiaCheck, Cotejo.info, EFE Verifica, Ecuador Chequea, Efecto Cocuyo, \#NoComaCuento (La Nación), La Silla Vacía, Mala Espina Check, Maldita.es, Newtral.es \\ \midrule
30 & El coronavirus fue fabricado en un laboratorio chino & Coronavirus was made in a Chinese lab & Chequeado, Ecuador Chequea, Estadão verifica \\ \bottomrule
\end{tabularx}%
}
\caption{Relation of hoaxes 1 - 30.}
\label{tab:hoaxes_1}
\end{table*}


\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabularx}{1.4\textwidth}{lXXX}

\toprule
\textbf{Id} & \textbf{Hoax (in Spanish)} & \textbf{Hoax (in English)} & \textbf{Fact-checkers} \\ \midrule
31 & La mascarilla causa hipoxia & Masks cause hypoxia & Agencia Ocote, Agência Lupa, Animal Político, Aos Fatos, Bolivia Verifica, Chequeado, ColombiaCheck, Cotejo.info, EFE Verifica, Ecuador Chequea, Efecto Cocuyo, La Silla Vacía, Maldita.es, Newtral.es, Verificado, Verificador (La República) \\ \midrule
32 & El eucalipto previene o cura el coronavirus & Eucalyptus prevents or cures coronavirus & AFP \\ \midrule
33 & El matico cura el coronavirus & Matico cures coronavirus & Bolivia Verifica \\ \midrule
34 & El biomagnetismo mata el coronavirus & Biomagnetism kills coronavirus & Bolivia Verifica, Maldita.es \\ \midrule
35 & La hoja de guayaba previene o cura el coronavirus & Guava leaf prevents or cures coronavirus & Animal Político, Bolivia Verifica, Maldita.es, Newtral.es \\ \midrule
36 & La NASA catalogó el dióxido de cloro como antídoto universal en 1988 & NASA catalogued chlorine dioxide as a universal antidote in 1988 & Animal Político \\ \midrule
37 & El vino previene o cura el coronavirus & Wine prevents or cures coronavirus & Chequeado, EFE Verifica, Maldita.es, Newtral.es \\ \midrule
38 & La mascarila causa la muerte por neumonía bacteriana & Masks cause death due to bacterial pneumonia & Maldita.es \\ \midrule
39 & La vitamina C previene o cura el coronavirus & Vitamin C prevents or cures coronavirus & AFP, Chequeado, EFE Verifica, Agência Lupa, Maldita.es, Verificado \\ \midrule
40 & La prueba de antígenos no sirve para la COVID-19 porque da positivo con Coca-Cola & Antigen tests are useless for COVID-19 because they test positive with Coca-cola & Maldita.es, Newtral.es \\ \midrule
41 & La homeopatía previene o cura el coronavirus & Homeopathy prevents or cures coronavirus & Chequeado, Mala Espina Check, Maldita.es, Periodismo de barrio / El Toque \\ \midrule
42 & La COVID-19, el MERS y el H1N1 coinciden con la instalación del 5G, 4G y 3G, respectivamente & COVID-19, MERS and H1N1 coincide with the installation of 3G, 4G and 5G, respectively & Poligrafo \\ \midrule
43 & Los indígenas protegen a los niños con hierbas y árboles frente a la COVID-19 & indigenous groups protect their children from COVID-19 with herbs and trees & Ecuador Chequea \\ \midrule
44 & Los mosquitos transmiten el coronavirus de contagiados & Mosquitoes transfer coronavirus from infected people & Maldita.es \\ \midrule
45 & Beber agua o sorbos previene o cura el coronavirus & Drinking or sipping water prevents or cures coronavirus & \#NoComaCuento (La Nación), AFP, Bolivia Verifica, ColombiaCheck, La Silla Vacía, Maldita.es, OjoPúblico \\ \midrule
46 & Mueren 55 personas en Estados Unidos tras vacunarse contra la COVID-19 & 55 people dead after being vaccinated against COVID-19 in the United States & EFE Verifica \\ \midrule
47 & Las mascarillas producen pleuresia y neumonía & Masks produce pneumonia and pleurisy & AFP \\ \midrule
48 & Las personas sanas llevan la mascarilla con la parte blanca hacia fuera para no contagiarse de COVID-19 & Healthy people wear their masks with the white part on the outside not to get COVID-19 & Newtral.es \\ \midrule
49 & El SARS-COV-2 no cumple los postulados de Koch, Rivers e Inglis para considerarlo enfermedad y coronavirus & SARS-COV-2 does not fulfill Koch, Rivers and Inglis' postulates in order to be considered as coronavirus and as a disease & EFE Verifica \\ \midrule
50 & Christine Lagarde dijo que los ancianos viven demasiado & Christine Lagarde said that the elderly live too long & Chequeado, ColombiaCheck, Ecuador Chequea, Maldita.es \\ \midrule
51 & La COVID-19 es una bacteria & COVID-19 is a bacteria & Animal Político, Chequeado, ColombiaCheck, La Silla Vacía, Maldita.es, Verificador (La República) \\ \midrule
52 & Galicia aprueba una ley para aislar a los positivos COVID-19 en campos de concentración & Galicia approves a law to aisle COVID-19 positives in concentration camps & Maldita.es \\ \midrule
53 & Las ondas electromagnéticas del 5G propagan el coronavirus & 5G electromagnetic waves spread coronavirus & Chequeado, Ecuador Chequea \\ \midrule
54 & La OMS rcomienda un test pulmonar para identificar el coronavirus & The WHO recommends a pulmonary test to detect coronavirus & EFE Verifica \\ \midrule
55 & Las pandemias tienen lugar cada 100 años & Pandemics take place every 100 years & AFP, Animal Político, ColombiaCheck, Verificador (La República) \\ \midrule
56 & El laboratorio de Wuhan tiene relación con Glaxo y Pfizer & Wuhan lab is related to Glaxo and Pfizer & Animal Político, Chequeado, La Silla Vacía, Maldita.es, Newtral.es \\ \midrule
57 & El coronavirus desaparece a los 27 grados & Coronavirus disappears at 27 degrees & Bolivia Verifica, Convoca, Agência Lupa \\ \midrule
58 & Hubo 17000 y 26000 muertes más en 2019 y 2018 respectivamente que en 2020 & There were 17000 and 26000 more deaths in 2019 and 2018 respectively than in 2020 & Maldita.es, Newtral.es \\ \midrule
59 & El polisorbato 80 de la vacuna contra la gripe causa coronavirus & Polysorbate 80 in the flu vaccines cause coronavirus & EFE Verifica, Maldita.es \\ \midrule
60 & Detienen a Charles Lieber por crear y vender el coronavirus & Charles Lieber arrested for creating and selling coronavirus & \#NoComaCuento (La Nación), AFP, Animal Político, Efecto Cocuyo, Agência Lupa, Mala Espina Check, Maldita.es, Newtral.es \\ \midrule
61 & En Israel no mueren por coronavirus gracias a una receta de limón y bicarbonato & No deaths in Israel due to coronavirus thanks to a recipe with lemon and bicarbonate & Newtral.es, Verificado \\ \bottomrule
\end{tabularx}%
}
\caption{Relation of hoaxes 31 - 61}
\label{tab:hoaxes_2}
\end{table*}




==> FacTeR-Check arxiv-2/tables/0-sick_summary.tex <==
\begin{table}[]
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}llcccc@{}}
\toprule
\multicolumn{1}{l}{}           & \multicolumn{1}{l}{\textbf{}}          & \textbf{Precision} & \textbf{Recall}       & \textbf{F1-score}     & \textbf{Support} \\ \midrule
\multirow{3}{*}{\textbf{Label}}   & \multicolumn{1}{l|}{\textit{CONTRADICTION}} & 0.9158 & 0.7486 & 0.8238 & 712  \\
                         & \multicolumn{1}{l|}{\textit{ENTAILMENT}}    & 0.8475 & 0.8946 & 0.8704 & 1404 \\
                         & \multicolumn{1}{l|}{\textit{NEUTRAL}}       & 0.8856 & 0.9022 & 0.8938 & 2790 \\ \midrule
\multirow{2}{*}{\textbf{Summary}} & \multicolumn{1}{l|}{\textit{Macro Avg.}}    & 0.8830 & 0.8484 & 0.8627 & 4906 \\
                         & \multicolumn{1}{l|}{\textit{Weighted Avg.}} & 0.8791 & 0.8777 & 0.8770 & 4906 \\ \midrule
\multicolumn{1}{c}{\textit{-}} & \multicolumn{1}{l|}{\textit{\textbf{Accuracy}}} & 0.8777             & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & 4906             \\ \bottomrule
\end{tabular}%
}
\caption{Results for the SICK test set.}
\label{tab:sick_v2}
\end{table}

==> FacTeR-Check arxiv-2/tables/0-sick_summary_v2.tex <==
\begin{table*}[]
\begin{tabularx}{\textwidth}{lrrYYYY}

%\begin{tabular}{lrrllll}
\hline
\textbf{Language} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{\textbf{}} &
  \textbf{Precision} &
  \textbf{Recall} &
  \textbf{F1-score} &
  \textbf{Support} \\ \hline
english & \multirow{3}{*}{Label}         & \multicolumn{1}{r|}{\textit{CONTRADICTION}} & 0.9158 & 0.7486 & 0.8238 & 712  \\
        &                                & \multicolumn{1}{r|}{\textit{ENTAILMENT}}    & 0.8475 & 0.8946 & 0.8704 & 1404 \\
        &                                & \multicolumn{1}{r|}{\textit{NEUTRAL}}       & 0.8856 & 0.9022 & 0.8938 & 2790 \\ \cline{2-7} 
        & \multirow{2}{*}{Summary}       & \multicolumn{1}{r|}{\textit{Macro Avg.}}    & 0.8830 & 0.8484 & 0.8627 & 4906 \\
        &                                & \multicolumn{1}{r|}{\textit{Weighted Avg.}} & 0.8791 & 0.8777 & 0.8770 & 4906 \\ \cline{2-7} 
 &
  \multicolumn{1}{c}{\textit{-}} &
  \multicolumn{1}{r|}{\textit{Accuracy}} &
  0.8777 &
  \multicolumn{1}{c}{-} &
  \multicolumn{1}{c}{-} &
  4906 \\ \hline
spanish & \multirow{3}{*}{Label}         & \multicolumn{1}{r|}{\textit{CONTRADICTION}} & 0.8511 & 0.7388 & 0.7910 & 712  \\
        &                                & \multicolumn{1}{r|}{\textit{ENTAILMENT}}    & 0.7446 & 0.9031 & 0.8162 & 1404 \\
        &                                & \multicolumn{1}{r|}{\textit{NEUTRAL}}       & 0.8797 & 0.8451 & 0.8461 & 2790 \\ \cline{2-7} 
        & \multirow{2}{*}{Summary}       & \multicolumn{1}{r|}{\textit{Macro Avg.}}    & 0.8251 & 0.8190 & 0.8178 & 4906 \\
        &                                & \multicolumn{1}{r|}{\textit{Weighted Avg.}} & 0.8369 & 0.8292 & 0.8296 & 4906 \\ \cline{2-7} 
        & \multicolumn{1}{c}{\textit{-}} & \multicolumn{1}{r|}{\textit{Accuracy}}      & 0.8292 & -      & -      & 4906 \\ \hline
\begin{tabular}[c]{@{}l@{}}inter\end{tabular} &
  \multirow{3}{*}{Label} &
  \multicolumn{1}{r|}{\textit{CONTRADICTION}} &
  0.8825 &
  0.8737 &
  0.8072 &
  1424 \\
        &                                & \multicolumn{1}{r|}{\textit{ENTAILMENT}}    & 0.7925 & 0.8989 & 0.8423 & 2808 \\
        &                                & \multicolumn{1}{r|}{\textit{NEUTRAL}}       & 0.8828 & 0.8586 & 0.8705 & 5580 \\ \cline{2-7} 
        & \multirow{2}{*}{Summary}       & \multicolumn{1}{r|}{\textit{Macro Avg.}}    & 0.8526 & 0.8337 & 0.84   & 9812 \\
        &                                & \multicolumn{1}{r|}{\textit{Weighted Avg.}} & 0.8569 & 0.8534 & 0.8533 & 9812 \\ \cline{2-7} 
        & \multicolumn{1}{c}{\textit{-}} & \multicolumn{1}{r|}{\textit{Accuracy}}      & 0.8534 & -      &  & 9812 \\ \hline
\end{tabularx}%

\caption{Results for the SICK test set. Spanish results are extracted from machine translations of the SICK test set. Interlingual results are made from pairing interchangeably Spanish and English prompts.}
\label{tab:sick_v2}
\end{table*}

==> FacTeR-Check arxiv-2/tables/keywords_queries_examples.tex <==
\begin{table*}
\centering
\resizebox{\linewidth}{!}{%\resizebox{\columnwidth}{!}{%
\begin{tabular}{ll} 
\toprule
\multicolumn{1}{c}{\textbf{Hoax}}                                                                   & \multicolumn{1}{c}{\textbf{Query}}                             \\ 
\midrule
La prueba de antígenos no sirve para la COVID-19 porque da positivo con Coca-Cola                   & (prueba AND antígeno AND covid-19 AND positivo AND coca-cola)  \\
Antigen tests are useless for COVID-19 because they test positive with CocaCola                     & (antigen AND test AND covid-19 AND cocacola)                   \\ 
\hline
En  Israel  no  mueren  por  coronavirus  gracias  a  una receta de limón y bicarbonato             & (coronavirus AND receta AND limón AND bicarbonato)             \\
No  deaths  in  Israel  due  to  coronavirus  thanks  to  a recipe with lemon and bicarbonate       & (israel AND coronavirus AND recipe AND lemon AND bicarbonate)  \\ 
\hline
La vacuna contra la COVID-19 causa esterilidad                                                      & (causa AND vacuna AND esterilidad AND contra AND covid-19)     \\
Pfizer vaccines cause sterility                                                                     & (pfizer AND sterility AND vaccines AND cause)                  \\ 
% \hline
% La  COVID-19,  el  MERS  y  el  H1N1  coinciden  conla instalación del 5G, 4G y 3G, respectivamente & (4g AND 5g AND 3g AND covid-19 AND h1n1)                       \\
% COVID-19,  MERS  and  H1N1  coincide  with  the installation of 3G, 4G and 5G, respectively         & (covid-19 AND h1n1 AND 3g AND 4g)                              \\
\bottomrule
\end{tabular}
}
\caption{Example of query building from English and Spanish hoaxes for searching through Twitter API. The queries are built concatenating the different keywords extracted with the AND logical operator.}
\label{table_keywords_example}
\end{table*}

==> FacTeR-Check arxiv-2/tables/tables_keyword_extraction.tex <==
 \begin{table}[htpb]
   \centering
        \resizebox{0.55\linewidth}{!}{%
              \centering
                \begin{tabular}{lccc} 
                \toprule
                \multicolumn{1}{c}{\multirow{2}{*}{Keyword Model}}  & \multicolumn{3}{c}{General}                          \\
                                                & Precision       & Recall          & F1-score         \\ 
                \hline
                RAKE Spanish                    & 0.4683          & 0.9503          & 0.6139           \\
                KeyBERT Multilingual            & 0.5694          & 0.7121          & 0.6200           \\
                \textbf{FactTeR-ChecKey Multilingual}  & \textbf{0.6283} & \textbf{0.8267} & \textbf{0.6988}  \\
                \bottomrule
                \end{tabular}
                }
                \vspace{2mm}
                \caption{Evaluation of the keywords extraction module in general purpose tasks.}
                \label{table:keys_general}
            \end{table}%
        
\begin{table}[htpb]
  \centering
\resizebox{0.68\linewidth}{!}{%
    \begin{tabular}{lccc} 
    \toprule
    \multicolumn{1}{c}{\multirow{2}{*}{Keyword Model}}       & \multicolumn{3}{c}{Twitter}                          \\
                                          & Precision       & Recall          & F1-score         \\ 
    \hline
    RAKE spanish + POS Tag Filter  small     & 0.5692          & 0.8851          & 0.6731           \\
    RAKE spanish + POS Tag Filter  medium     & 0.5703          & 0.8952          & 0.6794           \\
    RAKE spanish + POS Tag Filter  large     & 0.5707          & 0.8590          & 0.6653           \\
    \hline
    KeyBERT + POS Tag Filter small           & 0.6433          & 0.6572          & 0.6293           \\
    KeyBERT + POS Tag Filter medium           & 0.6442          & 0.6577          & 0.6317           \\
    KeyBERT + POS Tag Filter large           & 0.6483          & 0.6242          & 0.6107           \\
    \hline
    FactTeR-ChecKey + POS Tag Filter small          & 0.6436          & 0.7397          & 0.6657           \\
    FactTeR-ChecKey + POS Tag Filter medium          & 0.6852          & 0.7847          & 0.7104           \\
    \textbf{FactTeR-ChecKey + POS Tag Filter large} & \textbf{0.6888} & \textbf{0.7917} & \textbf{0.7149}  \\
    \bottomrule
    \end{tabular}
    }
    \vspace{2mm}
    \caption{Evaluation of the keywords extraction module in the Twitter API.}
    \label{table:keys_twitter}
\end{table} 

==> FacTeR-Check arxiv-2/tables/tables_semantic_similarity.tex <==
 
        % TABLE SPEARMAN STS
        \begin{table*}
            %\begin{subfigure}{\columnwidth}
            \centering
            \resizebox{\linewidth}{!}{%\resizebox{\columnwidth}{!}{%
            \begin{tabular}{lccccccccc} 
                \toprule
                \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Model}}}   & \multirow{2}{*}{\textbf{Dimensions}} & \multicolumn{2}{c}{\textbf{EN-EN}} & \multicolumn{2}{c}{\textbf{EN-ES}} & \multicolumn{2}{c}{\textbf{ES-ES}} & \multicolumn{2}{c}{\textbf{Avg}}  \\
                \multicolumn{1}{c}{}                         &                             & $r$   & $\rho$            & $r$   & $\rho$            & $r$   & $\rho$            & $r$   & $\rho$           \\ 
                \midrule
                MSTSb\_paraphrase-multilingual-MiniLM-L12-v2 & 348                         & 85.26 & 86.17             & 81.45 & 81.49             & 83.30 & 83.68             & 81.38 & 81.47            \\
                MSTSb\_stsb-xlm-r-multilingual               & 768                         & 84.21 & 85.10             & 82.65 & 83.04             & 83.20 & 83.83             & 81.75 & 82.09            \\
                MSTSb\_paraphrase-xlm-r-multilingual-v1      & 768                         & 84.80 & 85.59             & 82.90 & 83.19             & 83.41 & 83.71             & 82.39 & 82.60            \\
                MSTSb-paraphrase-multilingual-mpnet-base-v2  & 768                         & 86.80 & \textbf{87.40}    & 84.42 & 84.45             & 85.19 & \textbf{85.52}    & 83.48 & 83.59            \\
                Ensemble 2                                   & 1152                        & 85.90 & 86.72             & 83.68 & 83.87             & 84.39 & 84.67             & 83.25 & 83.41            \\
                Ensemble 3                                   & 1920                        & 86.34 & 87.13             & 84.18 & 84.34             & 84.86 & 85.14             & 83.67 & \textbf{83.84 }  \\
                Ensemble 4                                   & 2688                        & 85.73 & 86.59             & 84.16 & \textbf{84.53}    & 84.67 & 85.25             & 83.33 & 83.62            \\
                \bottomrule
            \end{tabular}
            }
            
            \caption{Spearman $\rho$ and Pearson $r$ correlation coefficient between the sentence representation from multilingual models and the gold labels for STS Benchmark test set.}
            \label{table:STS_single_models_test}
        \end{table*}
            
        % TABLE SPEARMAN STS PCA    
        \begin{table*}
            %\begin{subfigure}{\columnwidth}
            \centering
            \resizebox{\linewidth}{!}{%\resizebox{\columnwidth}{!}{%
            
            \begin{tabular}{lccccccccc} 
                \toprule
                \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Model + PCA}}} & \multirow{2}{*}{\textbf{Dimensions}} & \multicolumn{2}{c}{\textbf{EN-EN}} & \multicolumn{2}{c}{\textbf{EN-ES}} & \multicolumn{2}{c}{\textbf{ES-ES}} & \multicolumn{2}{c}{\textbf{Avg}}  \\
                \multicolumn{1}{c}{}                            &                             & $r$   & $\rho$            & $r$   & $\rho$            & $r$   & $\rho$            & $r$   & $\rho$           \\ 
                \midrule
                MSTSb\_paraphrase-multilingual-MiniLM-L12-v2    & 184                         & 84.92 & 85.71             & 81.04 & 81.04             & 83.08 & 83.28             & 81.03 & 81.02            \\
                MSTSb\_stsb-xlm-r-multilingual                  & 408                         & 84.35 & 85.11             & 82.84 & 83.17             & 83.39 & 83.89             & 81.85 & 82.08            \\
                MSTSb\_paraphrase-xlm-r-multilingual-v1         & 286                         & 84.79 & 85.50             & 82.73 & 82.97             & 83.38 & 83.58             & 82.23 & 82.39            \\
                MSTSb-paraphrase-multilingual-mpnet-base-v2     & 306                         & 86.69 & 87.27             & 84.21 & 84.28             & 84.93 & 85.19             & 83.20 & 83.28            \\
                Ensemble 2                                      & 347                         & 85.91 & 86.72             & 83.49 & 83.69             & 84.42 & 84.68             & 83.12 & 83.28            \\
                Ensemble 3                                      & 367                         & 86.64 & 87.55             & 84.50 & 84.80             & 85.24 & 85.72             & 83.85 & 84.21            \\
                Ensemble 4                                      & 429                         & 86.77 & \textbf{87.78}    & 85.00 & \textbf{85.52}    & 85.56 & \textbf{86.20}    & 84.24 & \textbf{84.71}   \\
                \bottomrule
            \end{tabular}
            }
            
            \caption{Spearman $\rho$ and Pearson $r$ correlation coefficient between the sentence representation from multilingual models with PCA dimenisonality reduction and the gold labels for STS Benchmark test set.}
            \label{table:STS_pca_models_test}
        \end{table*}

==> tables/0-sick_summary.tex <==
\begin{table}[]
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}llcccc@{}}
\toprule
\multicolumn{1}{l}{}           & \multicolumn{1}{l}{\textbf{}}          & \textbf{Precision} & \textbf{Recall}       & \textbf{F1-score}     & \textbf{Support} \\ \midrule
\multirow{3}{*}{\textbf{Label}}   & \multicolumn{1}{l|}{\textit{CONTRADICTION}} & 0.9158 & 0.7486 & 0.8238 & 712  \\
                         & \multicolumn{1}{l|}{\textit{ENTAILMENT}}    & 0.8475 & 0.8946 & 0.8704 & 1404 \\
                         & \multicolumn{1}{l|}{\textit{NEUTRAL}}       & 0.8856 & 0.9022 & 0.8938 & 2790 \\ \midrule
\multirow{2}{*}{\textbf{Summary}} & \multicolumn{1}{l|}{\textit{Macro Avg.}}    & 0.8830 & 0.8484 & 0.8627 & 4906 \\
                         & \multicolumn{1}{l|}{\textit{Weighted Avg.}} & 0.8791 & 0.8777 & 0.8770 & 4906 \\ \midrule
\multicolumn{1}{c}{\textit{-}} & \multicolumn{1}{l|}{\textit{\textbf{Accuracy}}} & 0.8777             & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & 4906             \\ \bottomrule
\end{tabular}%
}
\caption{Results for the SICK test set.}
\label{tab:sick_v2}
\end{table}

==> tables/keywords_queries_examples.tex <==
\begin{table*}
\centering
\resizebox{\linewidth}{!}{%\resizebox{\columnwidth}{!}{%
\begin{tabular}{ll} 
\toprule
\multicolumn{1}{c}{\textbf{Hoax}}                                                                   & \multicolumn{1}{c}{\textbf{Query}}                             \\ 
\midrule
La prueba de antígenos no sirve para la COVID-19 porque da positivo con Coca-Cola                   & (prueba AND antígeno AND covid-19 AND positivo AND coca-cola)  \\
Antigen tests are useless for COVID-19 because they test positive with CocaCola                     & (antigen AND test AND covid-19 AND cocacola)                   \\ 
\hline
En  Israel  no  mueren  por  coronavirus  gracias  a  una receta de limón y bicarbonato             & (coronavirus AND receta AND limón AND bicarbonato)             \\
No  deaths  in  Israel  due  to  coronavirus  thanks  to  a recipe with lemon and bicarbonate       & (israel AND coronavirus AND recipe AND lemon AND bicarbonate)  \\ 
\hline
La vacuna contra la COVID-19 causa esterilidad                                                      & (causa AND vacuna AND esterilidad AND contra AND covid-19)     \\
Pfizer vaccines cause sterility                                                                     & (pfizer AND sterility AND vaccines AND cause)                  \\ 
% \hline
% La  COVID-19,  el  MERS  y  el  H1N1  coinciden  conla instalación del 5G, 4G y 3G, respectivamente & (4g AND 5g AND 3g AND covid-19 AND h1n1)                       \\
% COVID-19,  MERS  and  H1N1  coincide  with  the installation of 3G, 4G and 5G, respectively         & (covid-19 AND h1n1 AND 3g AND 4g)                              \\
\bottomrule
\end{tabular}
}
\caption{Example of query building from English and Spanish hoaxes for searching through Twitter API. The queries are built concatenating the different keywords extracted with the AND logical operator.}
\label{table_keywords_example}
\end{table*}
